PATHoBot: A Robot for Glasshouse Crop Phenotyping and Intervention

We present PATHoBot an autonomous crop surveying and intervention robot for glasshouse environments. The aim of this platform is to autonomously gather high quality data and also estimate key phenotypic parameters. To achieve this we retro-fit an off-the-shelf pipe-rail trolley with an array of multi-modal cameras, navigation sensors and a robotic arm for close surveying tasks and intervention. In this paper we describe PATHoBot design choices made to ensure proper operation in a commercial glasshouse environment. As a surveying platform we collect a number of datasets which include both sweet pepper and tomatoes. We show how PATHoBot enables novel surveillance approaches by first improving our previous work on fruit counting by incorporating wheel odometry and depth information. We find that by introducing re-projection and depth information we are able to achieve an absolute improvement of 20 points over the baseline technique in an "in the wild" situation. Finally, we present a 3D mapping case study, further showcasing PATHoBot's crop surveying capabilities.

==> contribs/videoScript.tex <==
- Cover
	- video of trolley moving in the row
	script:
	In this work we present PATHoBot, A Robot for Glasshouse crop phenotyping and intervention.
   

- Stills of environment current sensing & camera array
    - Env still:
        script:
        Agricultural robotics is a rapidly moving research field, presenting multiple opportunities and challenges to automate processes with the aid of computer vision and machine learning. In particular, automated phenotyping from crop surveyed data. 
        
        In this work, we focus on surveying sweet pepper in a commercial glasshouse maintained by the Bonn university.
        In these images, you can see the crop chambers which have limited space and an example of how a person might use a handheld sensor on the fixed height trolley.
        These fixed height trolleys are used to drive along the heating pipes to perform intervention and close surveying tasks.
        script:
    
        We automated an off the shelf pipe-rail scissorlift platform and added an on-board computer running ROS, Navigation sensors, and a robot arm for intervention and close proximity surveying.
        We also added a custom multi-modal RGB-D camera array like the one shown in the image to capture Color, Depth and NIR data as they bring multiple benefits for estimating phenotypic indices.
        With this setup, we're able surveying entire crop rows on-the-fly as shown in this timelapse.
        
- timelapses from data collection?
    script:
    Where a whole chamber is scanned in under 50 minutes.
    This approach opens the door to more frequent estiamtion of phenotypic indices. 
    This platform is capable of autonomously driving through and surveying entire crop rows after it is manually snapped onto the glasshouse piperails by an operator.
    We decided to mount our camera array on a collapsible mast to avoid collisions with the obstacles present at the end of the rows.

- Explain detection approach
    The data gathered with this method enabled us to enhance our previous work on fruit counting of sweet pepper.
    The baseline method tracks fruit segmented by a neural network by superimposing old and current detections.
    Our improved approach exploits spatial-temporal information present in the datasets gathered by PATHoBot.
    We improve mask tracking by re-projecting detection masks to subsequent frames using depth from the cameras and motion information from the platform.
    We also use depth information to filter detections from outside of the surveyed row to avoid miss counts.
    As it can be seen in this extreme example, all baseline detections are from a far away row since there are no crops in the current surveyed row, so all detections are filter using depth information.
    This new approach manages to achieve approximately 20 points lower normalized counting error that the baseline.
	It is worth mentioning that the segmentation network was not trained to detect yellow pepper, however it manages to produce good and consistent detections.
	Here is another example of depth-wise detection filtering.
	
- Explain mapping approach
	script:
	We also show how this platforms allows us to 3D map a whole crop row from a single on-the-fly scan.
	We simply concatenate colored pointclouds from all RGB-D cameras and reference them to the same coordinate frame using the platform odometry and accounting for the camera extrinsics.
	Here you can see how crops are densely mapped, however occlusion produce un-mapped patches, and also data is noisy as this naive mapping approach only concatenates single depth measurement pointclouds.
	This naive mapping method can be improved by fusing all information (pointclouds and navigation sensors) to produce cleaner and more consistent maps.
	
